Service Registration, Indexing, Discovery & Selection; An Architectural Survey Toward a GenAI-Driven Future

The emergence of sixth-generation (6G) networks marks a paradigm shift: by unifying an edge-to-cloud computing continuum with ultra-high-performance networking, 6G will enable capabilities far beyond today's boundaries. As use-case diversity grows exponentially and user adoption drives traffic to unprecedented and highly dynamic levels, novel service orchestration mechanisms are indispensable. In this paper, we adopt an architectural viewpoint, examining Service Registration, Indexing, Discovery, and Selection (SRIDS) as fundamental elements of 6G service provision. We first establish the theoretical foundations of SRIDS in 6G by defining its core concepts, detailing its end-to-end workflow, reviewing current standardization efforts, and projecting its future design objectives, including reliability, scalability, automaticity and adaptability, determinism, efficiency, sustainability, semantic-awareness, security, privacy, and trust. We then perform a comprehensive literature review and gap analysis encompassing both existing surveys and recent research efforts, identifying conceptual and methodological gaps that hinder unified SRIDS in 6G. Next, we introduce a taxonomy that classifies SRIDS mechanisms into centralized, distributed, decentralized, and hybrid architectures, and systematically examine the relevant studies within each category. Each work is evaluated against the extracted design objectives. Building on these findings, we propose a hybrid architectural framework, combining centralized data management to ensure consistency and agility with distributed coordination to enhance scalability in emerging 6G use cases. The framework incorporates innovative technologies, such as Generative Artificial Intelligence (GenAI). We conclude by highlighting open challenges and suggesting directions for future research.

==> tables/tab3_t.tex <==
\begin{table*}[t]
\centering
\caption{Comparison of SRIDS architectures based on their functional role process type.}
\label{table:architecture_functionality_approaches}
\scriptsize
\begin{tabularx}{\textwidth}{p{2.1cm}X X X X}
\toprule
\textbf{SRIDS function} & \textbf{Centralized} & \textbf{Distributed} & \textbf{Decentralized} & \textbf{Hybrid} \\
\midrule
Service registration and indexing &
SLP-based (directory server for registration); DNS-based (hierarchical name resolution); Napster (central file index); broker-based (centralized registration); Detection Mesh &
Chord, Kademlia, Pastry, Kinaara (DHT for scalable indexing); IBSD (blockchain-based indexing) &
Gnutella, Freenet (peer-to-peer local registration) &
BitTorrent (tracker-assisted indexing with peer-to-peer distribution); eDonkey (centralized index + peer-to-peer search) \\

Service discovery and selection &
SLP-based (clients query directory server); broker-based (service matching); Detection Mesh (similarity match) &
CAN (structured overlays and selection mechanisms); IOTA (DAG-based coordination) &
Gnutella, SD-AMC (flooding-based discovery) &
Jini (lookup server + decentralized selection); Istio (service discovery via control plane with distributed execution) \\

Service routing and communication &
Kubernetes discovery (centralized coordination); broker-based (single control entity for routing) &
Kademlia, Pastry, Skip Graph, Cycloid, HandFan (self-organizing routing) &
Tree-based (hierarchical routing) &
Istio (proxy-based routing and hybrid coordination); CoAP-based approaches \\
\bottomrule
\end{tabularx}
\end{table*}

